Decomposition of complete tripartite graphs into 5-cycles using the graph adjacency matrix

The problem of decomposing a complete tripartite graph into 5-cycles was first proposed in 1995 by Mahmoodian and Mirzakhani and since then many attempts have been made to decompose such graphs into 5-cycles. Such attempts were partially successful but parts of the problem still remain open. In this paper, we investigate the problem deeper, decompose more tripartite graphs into 5-cycles, and introduce the Graph Adjacency Matrix (GAM) method for cycle decomposition in general. GAM method transforms the cycle decomposition problem to covering squares with certain polygons. This new formulation is easier to solve and enables us to find explicit decompositions for numerous cases that were not decomposed before.

==> hyperref/abbr.tex <==
\abbrdef{``}{\texorpdfstring{``}{\flqq}}
\abbrdef{''}{\texorpdfstring{''}{\frqq}}
\abbrdef{acroread}{\Program{AcrobatReader}}
\abbrdef{aux}{\File{.aux}}
\abbrdef{eg}{e.\,g\mbox{.}}
\abbrdef{gdi}{general document information}
\abbrdef{gs}{\Program{ghost\-script}}
\abbrdef{hyperref}{\Package{hy\-per\-ref}}
\abbrdef{hypbmsec}{\Package{hypbmsec}}
\abbrdef{ind}{\hbox{\texttt{ \ }}}
\abbrdef{isolatin1}{ISOLatin1}
\abbrdef{latex}{\LaTeX}
\abbrdef{latexe}{\texorpdfstring{\LaTeXe}{LaTeX2e}}
\abbrdef{mediabox}{/MediaBox}
\abbrdef{PD1}{PD1}
\abbrdef{pdf}{PDF}
\abbrdef{pdfdocencoding}{PDFDocEncoding}
\abbrdef{pdffile}{pdf file}
\abbrdef{pdfinfo}{\Program{pdfinfo}}
\abbrdef{pdfspec}{*pdf* specification}
\abbrdef{pdfstringdef}{\cms{pdfstringdef}}
\abbrdef{pdftex}{\Program{\pdfTeX}}
\abbrdef{perlscript}{perl script}
\abbrdef{plain}{plain}
\abbrdef{plaintex}{*plain*-*tex*}
\abbrdef{postscript}{PostScript}
\abbrdef{PU}{PU}
\abbrdef{sectioning}{section} % section?
\abbrdef{Sectioning}{Section}
\abbrdef{tex}{\TeX}
\abbrdef{texfile}{*tex* file}
\abbrdef{thumbpdf}{\Package{thumb\-pdf}}
\abbrdef{thumbpdf.pl}{\File{thumbpdf.pl}}
\abbrdef{toc}{\File{.toc}}
\abbrdef{unicode}{Unicode}
\abbrdef{winansiencoding}{WinAnsiEncoding}
\endinput


==> hyperref/docinfo.tex <==
\foilhead[-\baselineskip]{General Document Information}

%\begin{Nav}{\NavInfo\NavBack}%
\begin{Nav}{\NavInfo}%
  \newcommand{\tit}[1]{%
    \multicolumn{2}{@{}l@{}}{\textbf{#1}}\\[0.5ex]%
  }
  \newcommand{\longentry}[1]{%
    \multicolumn{2}{@{}l@{}}{#1}%
  }
  \noindent
  Application: search engines.

  \noindent
  \begin{minipage}[t]{.55\linewidth}
    \begin{tabular}[t]{@{}l>{\tt}l@{}}
    \tit{\hypertarget{info}{*hyperref* options:}}%
    Title:&\Blue{pdftitle}\\
    Subject:&\Blue{pdfsubject}\\
    Author:&\Blue{pdfauthor}\\
    Keywords:&\Blue{pdfkeywords}\\
    Creator:&\Blue{pdfcreator}\\
    Producer:&\Blue{pdfproducer}
    \end{tabular}
  \end{minipage}%
  \begin{minipage}[t]{.45\linewidth}
    \begin{tabular}[t]{@{}ll@{}}
      \tit{Times:}%
      Created:&\Green{/CreationDate}\\
      Modificated:&\Green{/ModDate}\\[1ex]
      \tit{Informations:}%
      \longentry{File name, file size}\\
      \longentry{*pdf* version}\\
      \longentry{Optimized(linearized)}
    \end{tabular}
  \end{minipage}

  \subfoilhead{Setting\texorpdfstring{ the general document information}{}}
  \begin{smallpar}\hypertarget{infoanw}{}%
  \noindent
  \Code{\cms{usepackage}\{hyperref\}}\par
  \vspace{-\parskip}
  \catcode`\^^M=5
  \verbatiminput{pdfinfo}
  \end{smallpar}
  \newpage

\end{Nav}


\iffalse
\begingroup
  \makeatletter
  \def\hyper@anchorstart#1\hyper@anchorend{}%
  \pdfbookmark[1]{\file{hyperref} options}{optinfo}
\endgroup
\fi

\endinput


==> hyperref/encoding.tex <==
\clearpage
\pdfbookmark[0]{Encodings}{enc}

\begingroup
\hypersetup{bookmarksopenlevel=2}


\subfoilhead[-\baselineskip]{Font encoding mechanism%
  \texorpdfstring{}{ of \abbr{latexe}}}

\noindent
\begin{tabular}{@{}l@{ }l@{ $\Rightarrow$ }l@{}}
plain-\TeX:& \code[green]<\ss>\ = \code[blue]<\char"19>&\Red{\ss}\\[1ex]
\LaTeXe:
  & \code<\fontencoding{OT1}\selectfont\char"19>&\Red{\ss}\\
  & \code<\fontencoding {T1}\selectfont\char"19>&\Red{\i}\\[0.5ex]
  & \code<\ss>\ = \code[blue]<\OT1-cmd \ss > \code[green]<\OT1\ss>&\Red{\ss}
\end{tabular}

\noindent
The font slot positions depend on the encoding:\\
\phantom{plain-\TeX: }\code[green]<\OT1\ss>\ = \code<\char"19>\\
\phantom{plain-\TeX: }\code[green]<\T1\ss>\phantom{\code<O>} =
  \code<\char"FF>\\
\phantom{plain-\TeX: }\code[green]<\?\ss>\phantom{\code<OT>} =
  \code<\UseTextSymbol{OT1}\ss>

%\begin{smallpar}
  \noindent
  \code<\> \code[blue]<OT1\ss>\ =
  \code<\csname > \code[blue]<OT1> \code<\string> \code[blue]<\ss>
    \code<\endcsname>
%\end{smallpar}


\subfoilhead[-\baselineskip]{PD1 encoding%
  \texorpdfstring{ (\abbr{pdfdocencoding})}{}}

\begin{itemize}
\def\1{\code[red]}%
\def\2{\code[blue]}\def\3{\Blue}%
\def\4#1{\Green{#1}\,=\,}%
\def\5{\Green}
\item Most names: \1<\text>%
    \3{\textsl{\textless glyph name\textgreater}}\\
    Examples:\quad
  \begin{tabular}[t]{@{}c@{\,=\,}l@{,\quad}c@{\,=\,}l@{}}
    \5\textregistered&\1<\text>\2<registered>&
    \5\textasciitilde&\1<\text>\2<asciitilde>
  \end{tabular}
\item Traditional *tex* and *latex* names.\\
    Examples:\quad
    \4\AE\2<\AE>,\quad
    \4\ss\2<\ss>
\item Accented characters.\\
    Examples:\quad
    \4{\"U}\2<\"U>,\quad
    \4{\c c}\2<\c c>,\quad
    \4{\r A}\2<\r A>~($\Leftarrow$\,\1<\AA>)
\item Escape octal sequences are the result:
%  \2<\textmu>\ (\Green{$\mu$}) $\Rightarrow$ \1<\265>
%  \2<\guillemotleft>\ (\Green{\guillemotleft}) $\Rightarrow$ \1<\253>
  \2<\textmu>\,$\Rightarrow$\,\1<\265>
\end{itemize}


\subfoilhead[-1.5\baselineskip]{PU encoding%
  \texorpdfstring{ (\abbr{unicode})}{}}

\begin{itemize}
\item[\frownie] Characters having catcodes 11 (letter) and 12 (other):\\
Checking each token, high memory and time consumption.
\item[\frownie] Ligatures: same as above.
\item[\frownie] Direct commands:\\
  Easier to implement, but each command must be redefined each time.
\item[\smiley] Commands of *latexe*'s fontencoding mechanism:\\
  Smallest memory consumption and fastest method.\\
  This method is used by package *hyperref*.
\end{itemize}


\subsubfoilhead[-\baselineskip]{Examples of \abbr{unicode} bookmarks}

\begingroup
\def\top#1{\vtop{\vskip0pt\hbox{#1}}}
\def\use#1{\top{\includegraphics[scale=1.2]{u0#1}}}
\centering
\begin{tabular}{@{}ll@{}}
\Blue{Greek}:&\Blue{Cyrillic}:\\
\use{3}&\use{4}\\
\end{tabular}
\par
\endgroup

\endgroup
\endinput


==> hyperref/ende.tex <==
\clearpage
\pdfbookmark[0]{Ende}{ende}

\subfoilhead[-1.5\baselineskip]{Zusammenfassung}
\begin{itemize}
  \item \Red{Dokumenteninformation}:
    \begin{itemize}
      \item \file{hyperref}-Optionen in \code[blue]<\hypersetup>.
    \end{itemize}
  \item \Red{Lesezeichen}:
    \begin{itemize}
      \item Vorsicht wegen fehlender Magenverarbeitung
      \item Vieles durch \code[blue]<hyperref.sty>\ automatisiert.
      \item Zusatzpaket \code[blue]<hypbmsec.sty>
      \item Besondere Effekte erfordern "`low level"'-Eingriffe.
    \end{itemize}
  \item \Red{Thumbnails}:
    \begin{itemize}
      \item
      Einfache Benutzerschnittstelle mit \code[blue]<thumbpdf>.
    \end{itemize}
\end{itemize}


\subfoilhead[-\baselineskip]{Bezugsquellen}

\begin{smallpar}
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{PDF-Spezifikation}:\hfill
\url{http://www.adobe.com/supportservice/devrelations/PDFS/TN/PDFSPEC.PDF}\\[\sep]
  \it&\Blue{pdf\TeX}: \url{http://www.tug.org/applications/pdftex/}\\
  &Win32: \url{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}\\
  &Dokumantation: \url{http://www.pragma-ade.nl/pdftex.htm}\\[\sep]
  \it&\Blue{hyperref}, \Blue{pd1enc.def}, \Blue{hyparen.sty}:
\url{ftp://ftp.dante.de/tex-archive/macros/latex/contrib/supported/hyperref/}\\[\sep]
  \it&\Blue{hypbmsec}: Noch per E-Mail, CTAN geplant.\\[\sep]
  \it&\Blue{thumbpdf}:\hfill
\url{ftp://ftp.dante.de/tex-archive/macros/pdftex/thumbpdf/}\\[\sep]
  \it&\Blue{ghostscript}:
\url{http://www.cs.wisc.edu/~ghost/} oder\\&
\url{http://ftp.dante.de/tex-archive/support/ghostscript/aladdin/}
\end{tabularx}
\endgroup
\end{smallpar}

\rightfooter{%
  \ifprint
  \else
    \NavFull\NavSep\NavPrev\NavSep\NavQuit
  \fi
}


==> hyperref/eurobm99.tex <==
%\includeonly{title,docinfo,strings,encoding,psd,hyperref,replace,pdfextra,thumb,summary,links,appendix}
%\includeonly{hyperref}

\begin{document}
\catcode`\*=\active
\include{title}
\include{docinfo}
\include{strings}
\include{encoding}
\include{psd}
\include{hyperref}
\include{replace}
\include{pdfextra}
\include{thumb}
\include{summary}
\include{links}
\include{appendix}
\end{document}


==> hyperref/hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump



==> hyperref/hyperref.tex <==
\foilhead{Bookmarks with package *hyperref*}
\begin{itemize}
\item Places for options.
\item Options for bookmarks.
\item Creating bookmarks.
\item Replacement methods.
\end{itemize}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead{Places for \texorpdfstring{*hyperref* }{}options}
\begin{enumerate}
\item Global: \Blue{\cms{documentclass}}\Code{[}\dots\Code{]} (*eg* driver)
\item Package: \Blue{\cms{usepackage}}\Code{[}\dots\Code{]}
\item Configuration file: \Blue{\File{hyperref.cfg}} with \cms{hypersetup}
\item After package has been loaded:
  \Blue{\cms{hypersetup}}\Code{\{}\dots\Code{\}}\\
  (*eg* *pdf* information options)
\end{enumerate}


\subfoilhead[-1.5\baselineskip]{Bookmark options}

\begingroup
  \def\sep{0.5ex}
  \noindent
  \Red{\Option{bookmarks}}: Make bookmarks
    (default: \Green{\Value{true}}).\\[\sep]
  \Red{\Option{bookmarksnumbered}}: Put section numbers in bookmarks
    (\Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopen}}: Open up bookmark tree
     (default: \Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopenlevel}}: Level, to which bookmarks are
     open.\\[\sep]
  \Red{\Option{pdfpagemode}}: How document starts when opened
     (default: \Green{\Value{None}}):
  \begingroup
    \mbox\qquad\Blue{\Option{None}}: Neither outlines nor thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{UseOutlines}}, \Blue{\Option{UseThumbs}}:
      Outlines, thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{FullScreen}}: Full-screen mode.\\[\sep]
  \endgroup
  \Red{\Option{unicode}}: Bookmarks in *unicode*
     (\Green{\Value{false}}). After package has been\\
     \mbox\qquad loaded, it switches between *unicode* and *pdfdocencoding*.
\endgroup


\subfoilhead[-0.5\baselineskip]{%
  \texorpdfstring{Bookmarks by \abbr{sectioning}}{\abbr{Sectioning}} %
  commands
}
\label{sec:bmbysec}

\begin{itemize}
\item Automatically addition of bookmarks by:
      \begin{itemize}
      \item \cms{part}, \cms{chapter}, \cms{section}, \cms{subsection}, \dots
      \item \cms{addcontentsline}
      \end{itemize}
\item Help file \Blue{\Code{\textsl{\cms{jobname}}.out}}:
      \begin{itemize}
      \item It is written in the \Green{first} run.
      \item The bookmarks are set in the \Green{second} run.
      \item There is \Green{\emph{no}} ``rerun'' warning.
      \end{itemize}
\end{itemize}


\subfoilhead{Tree structure\texorpdfstring{ of bookmarks}{}}

\begin{itemize}
\item Subentries must be added to \Blue{direct} ancestores,
      \Blue{not} grandparents.
\item If an intermediate level is omitted, the leaf starts \Blue{leftmost}:
      \begin{quote}
        \def\sub{\Red{\ensuremath{\rightarrow}}}%
        \def\ver{\Red{\ensuremath{\|}}}%
        \begin{tabular}{@{}lll@{}}
        &\Blue{table of contents}&\Blue{bookmarks}\\
        \hline
        \cms{part}\Code{\{I\}}&\ver{Part I}&\ver{main entry}\\
        \cms{chapter}\Code{\{5\}}&%
          \ver\sub{Chapter I.5}&\ver\sub{subentry}\\
        \cms{subsection}\Code{\{1\}}&
          \ver\sub\sub\sub{Subsection I.5.0.1}&\ver{main entry}\\
        \end{tabular}
      \end{quote}
\end{itemize}


\subfoilhead[-\baselineskip]{\texorpdfstring{Creating bookmarks with }{}\cms{pdfbookmark}}

\begin{itemize}
\item The bookmarks of *sectioning* commands have an \Red{level} number:
      \par\noindent
      \begin{tabular}{@{}lc@{ }c@{ }c@{ }c@{ }c@{}}
      documentclass&\cms{part}&\cms{chapter}&%
        \cms{section}&\cms{subsection}&\dots\\
      \Class{book}/\Class{report}:&\Red{\llap{$-$}1}&%
        \Red0&\Red1&\Red2&\dots\\
      \Class{article}:&\Red0&&\Red1&\Red2&\dots\\
      \end{tabular}
\item Syntax of \Blue{\cms{pdfbookmark}} (default for level: \Red{0}):
      \begin{quote}
        \Blue{\cms{pdfbookmark}}%
          \Code{[\Red{\emph{level}}]\{\emph{bookmark text}\}%
            \{\Green{\emph{anchor name}}\}}
      \end{quote}
\item \Blue{\cms{currentpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level}
\item \Blue{\cms{subpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level + 1}
\end{itemize}


\subsubfoilhead[-\baselineskip]{Using anchors%
  \texorpdfstring{ with \cms{pdfbookmark}}{}%
}

\begin{itemize}
\item An \Green{anchor name} consists of the argument and
      the level:
      \begin{quote}
        \Blue{\cms{pdfbookmark}}\Code{[\Red0]\{Titlepage\}\{\Green{tit}\}}%
          \Code{\commentchar\ }anchor: \Code{\Green{tit}.\Red0}
      \end{quote}
\item The bookmark can point to another \Green{target} (\Green{anchor}):
      \begin{quote}\small
        \cms{hypertarget}\Code{\{\Green{place.}\Red{1}\}\{\}}
      \end{quote}
      Redirecting the bookmark to the previous defined \Green{target}:
      \begin{quote}\small
        \cms{begingroup}\\
        *ind*\cms{makeatletter}\\
        *ind*\cms{def}\cms{hyper@anchorstart}\Code{ \#1}%
          \cms{hyper@anchorend}\Code{\{\}\%}\\
        *ind*\Blue{\cms{pdfbookmark}}\Code{[\Red1]\{Go to the place\}\{\Green{place}\}\%}\\
        \cms{endgroup}
      \end{quote}
\end{itemize}

\endgroup
\endinput


==> hyperref/links.tex <==
\subfoilhead[-\baselineskip]{Links}

\begin{Nav}{\NavBookmarks\NavQuit}

\begin{smallpar}
\let\Blue\empty
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{*pdfspec*} (version 1.3):\newline
    \link{http://partners.adobe.com/asn/developer/PDFS/TN/PDFSPEC.PDF}%
    \tabularnewline[\sep]
  \it&\Blue{*pdftex*}:
    \begingroup
      \settoheight{\dimen0}{\mbox{\^e}}%
      \settoheight{\dimen1}{\mbox{e}}%
      \addtolength{\dimen0}{-\dimen1}%
    (H\`an Th\rlap{\raise\dimen0\hbox{\'{}}}\^e Th\`anh):
    \endgroup
    \newline
    \link{http://www.tug.org/applications/pdftex/}\newline
    Win32: \link{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}%
    \tabularnewline[\sep]
  \it&\Blue{*hyperref*} (Sebastian Rahtz):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/hyperref/}%
    \newline
    Test versions:\newline
    \link{http://www.tug.org/applications/hyperref/hyperref.zip}
    \tabularnewline[\sep]
  \it&\Blue{*hypbmsec*} (Heiko Oberdiek):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/oberdiek/}%
    \tabularnewline[\sep]
  \it&\Blue{*thumbpdf*} (Heiko Oberdiek):\newline
    \link{ftp://ctan.tug.org/tex-archive/macros/pdftex/thumbpdf/}%
\end{tabularx}
\endgroup
\end{smallpar}

%\SetNav{\NavFull\NavSep\NavPrev\NavSep\NavQuit}
\end{Nav}

\endinput


==> hyperref/navbook.tex <==
\newcommand{\bmaction}[3][0]{%
  \begingroup
    \pdfstringdef\x{#3}%
    \pdfoutline user {<</S /Named /N /#2>>} count #1 {\x}%
  \endgroup
}
\bmaction[-3]{NOP}{Navigation}
  \bmaction[2]{FullScreen}{Full-screen}
    \bmaction{PageOnly}{Page only}
    \bmaction{ShowThumbs}{Thumbnails}
  \bmaction[6]{NOP}{Selecting pages}
    \bmaction{PrevPage}{Previous page}
    \bmaction{NextPage}{Next page}
    \bmaction{GoBack}{Go back}
    \bmaction{GoForward}{Go forward}
    \bmaction{FirstPage}{First page}
    \bmaction{LastPage}{Last page}
  \bmaction[2]{GeneralInfo}{General document information}
    \bmaction{ShowHideMenuBar}{Menu bar}
    \bmaction{ShowHideToolBar}{Tool bar}

\endinput


==> hyperref/pdfextra.tex <==
\foilhead{Additional features of \abbr{pdf} format}
\noindent
Hyperref does not support all possibilities of *pdf* format, e.\,g.:
\begin{itemize}
  \let\Blue\empty
  \item \Blue{\Code{/CreationDate}} and \Blue{\Code{/ModDate}}.
  \item \Blue{Bookmarks} with \Blue{other functions}.
\end{itemize}
The following examples uses commands of \empty{*pdftex*}.

\subfoilhead{Bookmarks with other functions}
\begin{Nav}{\NavBookmarks\NavPage}

\begin{itemize}
  \item Menu functions of AcrobatReader, sound, video, \dots
  \item *pdftex* low level command:\\[1ex]
        \code[red]<\pdfoutline>\ \emph{\code<action>}\
        \code<count>\ \emph{\code[blue]<n>}\
        \code<{>\emph{\code<text>}\code<}>
        \begin{itemize}
          \item
            The absolute value of \emph{\code[blue]<n>}\ is the
            count of the direct subentries.
          \item
            If \emph{\code[blue]<n>}\ is negative, the
            subentries are closed.
        \end{itemize}
\end{itemize}


\subfoilhead{Link to external file}
\noindent
The *pdfspec* contains the possible actions on page 96.\\
At last a bookmark that points to that page:
\begingroup
  \edef\({\string(}
  \edef\){\string)}
\begin{verbatim}
$Blue(\pdfoutline)
  user {<<$Green(/S /GoToR /F $(pdfspec.pdf$) /D [95 /Fit])>>}
  count 0 {$empty(Description of actions)}
\end{verbatim}
\endgroup

\end{Nav}

\endinput


==> hyperref/pdfinfo.tex <==
\hypersetup!{%
  pdftitle!    = {PDF information and navigation elements},
  pdfsubject!  = {Slides for talk at EuroTeX'99 in Heidelberg},
  pdfkeywords! = {pdf, hyperref, bookmarks, thumbnails},
  pdfauthor!   = {\textcopyright\ Heiko Oberdiek},
  pdfcreator!  = {\LaTeX\ with package \flqq hyperref\frqq},
  pdfproducer! = {pdfeTeX-0.\the\pdftexversion\pdftexrevision},
}
\pdfinfo!{/CreationDate! (D:19990909000000-01'00')}

==> hyperref/psd.tex <==

\foilhead[-\baselineskip]{\cms{pdfstringdef}%
  \texorpdfstring{  converts \abbr{tex} to \abbr{pdf} strings}{}}

\noindent
Syntax: \Blue{\cms{pdfstringdef}}\Code{\{\emph{\cms{command}}\}%
    \{\emph{*tex* string}\}}

\begin{enumerate}
\item Selecting the encoding *PD1* or *PU*.
\item Redefinitions of many commands, so that they
      produce correct\\
      results or do not harm.
\item Expansion of the string.
\item Token checks and removal of forbidden tokens with 
      comprehensive\\ 
      warnings.
\end{enumerate}


\subfoilhead[-.5\baselineskip]{Redefinitions%
  \texorpdfstring{ by \cms{pdfstringdef}}{}}
\begin{itemize}
\item Redefinitions to get correct results, *eg*:
      \begin{itemize} 
      \item Glyph commands: \cms{\{}, \cms{\%}, \cms{space}, \cms{dots},
            \dots
      \item Logos: \cms{TeX}, \cms{LaTeX}, \cms{MF}, \dots
      \end{itemize}
\item Many tokens are removed silently, *eg*:
      \begin{itemize}
      \item *latex* commands: \cms{label}, \cms{index}, 
           \cms{textbf}, \dots
      \item Stomach tokens: curly group braces, \cms{relax} (\cms{protect}), 
            \dots
      \end{itemize}
\item The behaviour of \cms{xspace} is simulated.
\end{itemize}

\endinput


==> hyperref/replace.tex <==
\foilhead{Replacement methods}

\begin{itemize}
%\item \code[blue]<\texorpdfstring>\ provides an alternative.
\item \Blue{\cms{texorpdfstring}} choices one of its arguments:\\
      a *tex* or a *pdf* string.
\item \code[blue]<\pdfstringdefPreHook>\ is a place for redefining commands.\\
      Additions are made by \code[blue]<\pdfstringdefDisableCommands>.
\item Package \Blue{*hypbmsec*} extends the \code<\section>\ commands.
\end{itemize}


\subfoilhead{\cms{texorpdfstring} method}
\noindent
Syntax: \Red{\cms{texorpdfstring}}%
        \Green{\Code{\{*tex* string\}}}%
        \Blue{\Code{\{*pdf* string\}}}

\noindent
Example:

\noindent
  \cms{section}\Code{\{}\Red{\cms{texorpdfstring}}%
  %\Code{\emph{\%}}%
  \Green{\Code{\{H\$\_2\$O\}}}%
  %\Code{\emph{\%}}%
  \Blue{\Code{\{Water\}}}%
  %\Code{\emph{\%}}%
  \Code{\}}


\subfoilhead[-1\baselineskip]{Hook for private macro redefinitions}

\begin{itemize}
\item \Red{\cms{pdfstringdefPreHook}} is called, before expanding the string.
\item \Red{\cms{pdfstringdefDisableCommands}} adds user redefinitions to\\
      \cms{pdfstringdefPreHook}

  \Blue{\cms{pdfstringdefDisableCommands}}\Code{\{\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{textcolor}\}[1]\{\#1\}\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{url}\}}\Code{\{}\empty{\cms{pdfstringdefwarn}}%
    \Code{\{\cms{url}\}}\Code{\}\commentchar}\\
  *ind*\cms{let}\cms{textcolor}\cms{@gobble}\\
  \Code{\}}
\item \Red{\cms{pdfstringdefwarn}} prints a warning message.
\end{itemize}


\subfoilhead[-\baselineskip]{Package \Package{hypbmsec}}

\begin{itemize}
\item The syntax of \cms{section} commands is extended:
      \begin{itemize}
      \item Second optional bookmark argument.
      \item Bookmark in parentheses.
      \end{itemize}
\item Syntax:
  \def\txt{\Blue{\textsl{text}}}%
  \def\toc{\Green{\textsl{toc/head}}}%
  \def\out{\Red{\textsl{bookmark}}}%
  \settowidth{\dimen0}{\toc}%
  \settowidth{\dimen1}{\out}%
  \addtolength{\dimen1}{-\dimen0}%
  \setlength{\dimen1}{.5\dimen1}%
  \edef\toc{\noexpand\Green{\noexpand\textsl{toc%
    \noexpand\hspace{\the\dimen1}/\noexpand\hspace{\the\dimen1}head}}}%
  \settowidth{\dimen0}{\textbf{]\{}}%
  \settowidth{\dimen1}{ = }%
  \addtolength{\dimen0}{-\dimen1}%
  \setlength{\dimen0}{-.5\dimen0}%
  \edef\xsp{\noexpand\hspace{\the\dimen0}}%
  \def\({\textbf{(}\,}%
  \def\){\,\textbf{)}}%
  \def\[{\textbf{[}\,}%
  \def\]{\,\textbf{]}}%
  \def\{{\textbf{\orgbraceleft}\,}%
  \def\}{\,\textbf{\orgbraceright}}%
  \def\section{\cms{section}}%
  \def~{ = }%
  \begin{tabular}[t]{@{}l@{ }c@{}c@{}c@{}c@{}c@{}l@{}}
    \section&\{&\toc&~&\out&~&\txt\}\\
    \section&\[&\toc&~&\out&\]\,\{&\txt\}\\[1ex]
    \section&\[&\toc&\]\,\[&\out&\]\,\{&\txt\}\\[1ex]
    \section&\(&\out&\)\,\{&\toc&~&\txt\}\\
    \section&\[&\toc&\]\,\(&\out&\)\,\{&\txt\}\\
    \section&\(&\out&\)\,\[&\toc&\]\,\{&\txt\}\\
  \end{tabular}
\end{itemize}


\endinput

The next version of package *hypbmsec* will know the
option \Blue{\Option{startotoc}}:
The starred *sectioning* commands are included in the table
of contents and in the outline tree automatically.
For options \Blue{\Option{infix}} and \Blue{\Option{prefix}}
see \secref{sec:addcontentsline}.

\endinput


==> hyperref/strings.tex <==
\clearpage
\pdfbookmark[0]{Strings}{string}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead[-\baselineskip]{\abbr{pdf} strings}

\begin{itemize}
\item Examples, where *pdf* strings are used:
      \begin{quote}
      Bookmark names, information dictionaries, text annotations
      \end{quote}
\item *pdf* strings follow the *postscript* rules:
      \begin{itemize}
      \item Delimited by parentheses: \Code{\Blue{(}This is a string\Blue{)}}
      \item Escape sequences for white space, \Blue{\cms{(}}, \Blue{\cms{)}},
            \Blue{\cms{}\cms{}};\\
            octal notation, *eg*: `\"a\"o\"u\ss' = 
            \Code{(}\Blue{\cms{344}\cms{366}\cms{374}\cms{337}}\Code{)}
      \end{itemize}
\item 
%      $\vcenter{\mbox{%
        \begin{tabular}[t]{@{}l@{ }l@{}}
          \Blue{*pdfdocencoding*}:&8bit, superset of *isolatin1*\\
          \Blue{*unicode*}:&16bit, *acroread* version $\ge$ 4\\
        \end{tabular}%
%      }}$ 
\end{itemize}


\clearpage
\pdfbookmark[1]{\abbr{tex} strings}{strings}

\subsubfoilhead[-.5\baselineskip]{Digestion of \abbr{tex}}

\begingroup
\newenvironment{organ}[2]{%
  \begin{minipage}[t]{\linewidth}%
    \vspace{#2}%
    \begin{tabbing}%
      \begin{tabular}{@{\textbullet\ }l@{}}
        \multicolumn{1}{@{}l@{}}{%
%          \phantom{\textbullet\ }%
          \textbf{\large\Blue{#1}}}\\[0.5ex]
}{
      \end{tabular}%
    \end{tabbing}%
  \end{minipage}%
}

\makeatletter
\let\fbox\@firstofone

\noindent
\fbox{%
\begin{organ}{Eyes}{0pt}
  Reading input lines\\
  Catcodes are set
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Mouth}{2\baselineskip}
  Forming tokens\\
  Expansion of macros
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Stomach}{4\baselineskip}
  Assignments\\
  Typesetting
\end{organ}}%

\endgroup


\subsubfoilhead[-.5\baselineskip]{Differences between mouth and stomach}

\noindent
\begin{tabular}{@{}lll@{}}
  &\Blue{\textbf{mouth}}&
   \Blue{\textbf{stomach}}\\[1ex]
``zero'':& \code<\empty>&\code<\relax>\\[0.5ex]
\code<{...}>:&parameter&group\\[0.5ex]
variable:&read and check&assignments\\[0.5ex]
fonts:&--&different fonts and encodings\\
&&ligatures\\[0.5ex]
Commands:&\code<\string>, \code<\number>&\code<\def>, \code<\hbox>, \code<$>\\
&\code<\if>, \code<\the>&\code<\begingroup>, \code<\special>
\end{tabular}


\subfoilhead[-.5\baselineskip]{\abbr{tex} into \abbr{pdf} strings}

\begin{itemize}
\item Reusing the argument of *sectioning* commands (*tex* string)\\
      for the bookmarks (*pdf* strings).
\item Limitations because of missing stomach digestion:
      \begin{itemize}
      \item No manipulation of boxes, no mathematics, no colors, \dots
      \item No change of fonts or encodings, no ligatures.
      \item No assignments (\cms{xspace} uses \cms{futurelet}).
      \item Unexpandable commands appear verbatim.
      \end{itemize}
\end{itemize}


\endgroup
\endinput

==> hyperref/summary.tex <==
\clearpage
\pdfbookmark[0]{End}{ende}

\subfoilhead[-1.5\baselineskip]{Summary}
\begin{itemize}
  \item \Red{General document information}:
    \begin{itemize}
      \item Options in \code[blue]<\hypersetup>\
            after \cms{usepackage}\Code{\{hyperref\}}.
    \end{itemize}
  \item \Red{Bookmarks}:
    \begin{itemize}
      \item Automatically added by \Blue{*hyperref*}.
      \item \Blue{Oral expansion}, no stomach commands (exceptions).
      \item Replacement methods: \code[blue]<\texorpdfstring>,\\
            \code[blue]<\pdfstringdefDisableCommands>, and
            \Blue{*hypbmsec*}.
      \item Low level commands only for special effects.
    \end{itemize}
  \item \Red{Thumbnails}: Automatically added by \Blue{*thumbpdf*}.
\end{itemize}


==> hyperref/thumb.tex <==

\foilhead{Thumbnails}
\begin{Nav}{\NavThumbnails\NavBookmarks}
\thisthumb{zurueck}
\begin{itemize}
  \item Another method for navigation:
    \begin{itemize}
      \item Choosing pages.
      \item Selecting page areas.
    \end{itemize}
  \item Contents:
    \begin{itemize}
      \item Thumbnail sketches of the pages.
      \item Other pictograms, symbols, \dots
      \item Empty.
    \end{itemize}
\end{itemize}


\subfoilhead{Adding thumbnails with \abbr{thumbpdf}}
\thisthumb{weiter}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Nummer[#1]#2{\makebox(20,60)[#1]{%
    \vphantom{Hg}%
    $\smash{%
      \textsf{\textcircled{\vphantom{\large#2}\Blue{\small#2}}}%
    }$%
  }}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \begin{picture}(670,250)
    % Dateinamen
    \put(80,0){\FileBox{thumbdta.tex}}
    \put(80,100){\FileBox{\emph{jobname}.pdf}}
    \put(80,200){\FileBox{\emph{jobname}.tex}}
    \put(470,200){\FileBox{\Red{\emph{jobname}.pdf}}}
    % Pfeile
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(260,220){\line(1,0){210}}
    \put(470,220){\Right}
    \put(260,20){\line(1,0){105}}
    \put(365,20){\line(0,1){160}}
    \put(365,180){\Up}
    % Nummern
    \put(190,140){\Nummer[l]{1}}
    \put(190,40){\Nummer[l]{2}}
    \put(280,230){\Nummer[lb]{3}}
    % Programme
    \put(-10,40){\ProgBox[r]{*thumbpdf*}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(285,230){\ProgBox[b]{*pdftex*}}
    \put(285,150){\ProgBox[t]{\Code{thumbpdf.sty}}}
  \end{picture}
\endgroup

\subfoilhead[-\baselineskip]{How \abbr{thumbpdf} works}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \def\Left{\makebox(0,0)[l]{\LEFTarrow}}%
  \begin{picture}(650,340)
    % Dateinamen
    \put(80,0){\FileBox{\Red{thumbdta.tex}}}
    \put(80,100){\FileBox{thumbdta.pdf}}
    \put(80,200){\FileBox{thumb\emph{???}.png}}
    \put(80,300){\FileBox{\emph{jobname}.pdf}}
    \put(420,150){\FileBox{thumbopt.tex}}
    \put(420,240){\FileBox{\emph{other images}}}
    % Pfeile
    \put(170,300){\line(0,-1){60}}
    \put(170,240){\Down}
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(360,170){\line(1,0){60}}
    \put(360,170){\Left}
    \put(510,240){\line(0,-1){50}}
    \put(510,190){\Down}
    % Programme
    \put(-10,40){\ProgBox[r]{\textsf{perl}}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(190,140){\ProgBox[l]{\Code{thumbpdf.tex}}}
    \put(-10,240){\ProgBox[r]{*gs*}}
  \end{picture}
\endgroup


\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfoilhead{Thumbnails and *pdftex*}
\begin{itemize}
\item There is no direct support.
\item \code[blue]<\pdfimage> (*pdftex* versions below 0.14):
  \begin{itemize}
    \item[$+$] Image works as thumbnail.
    \item[$-$] No access to the image object number.
    \item[$-$] Image is on the page, must be
               moved out of the page.
  \end{itemize}
\item Low level commands
  \code[blue]<\pdfobj>\ and \code[blue]<\pdflastobj>\ are possible.
\end{itemize}

\clearpage
\pdfbookmark[1]{Project *thumbpdf*}{thumbpdf}
\subsubfoilhead[-\baselineskip]{Solution\texorpdfstring{ of project *thumbpdf*}{}}

\begin{enumerate}
  \item Generating the thumbnails \Blue{\file{thumb???.png}} by \Red{*gs*}.
  \item \Red{*pdftex*} runs \Red{\file{thumbpdf.tex}},
        thumbnails included by \code[blue]<\pdfimage>.
  \item The perl script \Red{\file{thumbpdf.pl}} reads
        \Blue{\file{thumbpdf.pdf}} and writes\\
        the object data in a *tex*
        readable form \Blue{\file{thumbdta.tex}}.
  \item Package \Red{\file{thumbpdf.sty}} inputs \Blue{\file{thumbdta.tex}},
        that contains the\\
        thumbnails as *pdf* objects (\code[blue]<\pdfobj>).
  \item The object numbers of the thumbnails (\code[blue]<\pdflastobj>)
        are added\\
        to the page attributes (\code[blue]<\pdfpageattr>).
\end{enumerate}


\subsubfoilhead[-.5\baselineskip]{User interface\texorpdfstring{ of *thumbpdf*}{}}

\begin{itemize}
  \def\master{\textsl{master}}%
  \item Command lines (\file{\master.tex} inputs \file{thumbpdf.sty}):
    \begin{enumerate}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
      \item \Blue{\texttt{thumbpdf \master}}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
    \end{enumerate}
  \item Another program than *gs* can be used:
    \begin{enumerate}
      \item[2a.] \Blue{\texttt{\textsl{ProgramThatGeneratesThumbnails} \master.pdf}}
      \item[2b.] \Blue{\texttt{thumbpdf}}
    \end{enumerate}
\end{itemize}

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subfoilhead[-\baselineskip]{Other images as thumbnails}

\begin{itemize}
\item With \Blue{\cms{thumb}} other images are declared as
      thumbnails in the\\ 
      optional file \Blue{\file{thumbopt.tex}}.
\item \Blue{\cms{thisthumb}} sets the thumbnail for the current page.
\end{itemize}
\begingroup
  \let\Red\Green
  \centering
  \begin{tabular}{@{}l@{\quad$\rightarrow$\quad}l@{}}
    \multicolumn{1}{@{}l}{\empty{\File{thumbopt.tex}}}&%
      \File{\emph{jobname}.tex}\\
    \hline
    \empty{\cms{thumb}}\Code{\{\Red{one}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
    \empty{\cms{thumb}}\Code{\{\Red{one.png}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one.png}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{two}]\{one\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{two}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{one}]\{./extras/one.png\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
  \end{tabular}
  \par
\endgroup

\end{Nav}

\endinput


==> hyperref/thumbopt.tex <==
\thumb[zurueck]{addthumb/thumb001.png}
\thumb[weiter]{addthumb/thumb002.png}


==> hyperref/title.tex <==
\pdfbookmark[0]{Beginning}{anfang}
\pdfbookmark[1]{Title}{title}

%\date{21st September 1999}% EuroTeX'99
\date{13rd October 1999}% first release for hyperref
\title{*pdf* information and navigation elements with
       hyperref, *pdftex*, and thumbpdf}
\author{Heiko Oberdiek\\\Email{oberdiek@ruf.uni-freiburg.de}}

\begingroup
  \LogoOff\aftergroup\LogoOn
  \Restriction{\unskip\centerline{\NavStart}}%
  \aftergroup\Restriction\aftergroup\empty
  \maketitle
  \begin{abstract}
    \noindent
    Additional possibilities for information and navigation through
    paper-less on-line documents that offer the PDF format.
  \end{abstract}
  \newpage
\endgroup

\subfoilhead{Subjects}
\begin{itemize}
\item General document information\hfill*hyperref*
\item Bookmarks/outlines\hfill*hyperref*
\item Thumbnails\hfill*thumbpdf*
\end{itemize}

\endinput


==> without review/hyperref/abbr.tex <==
\abbrdef{``}{\texorpdfstring{``}{\flqq}}
\abbrdef{''}{\texorpdfstring{''}{\frqq}}
\abbrdef{acroread}{\Program{AcrobatReader}}
\abbrdef{aux}{\File{.aux}}
\abbrdef{eg}{e.\,g\mbox{.}}
\abbrdef{gdi}{general document information}
\abbrdef{gs}{\Program{ghost\-script}}
\abbrdef{hyperref}{\Package{hy\-per\-ref}}
\abbrdef{hypbmsec}{\Package{hypbmsec}}
\abbrdef{ind}{\hbox{\texttt{ \ }}}
\abbrdef{isolatin1}{ISOLatin1}
\abbrdef{latex}{\LaTeX}
\abbrdef{latexe}{\texorpdfstring{\LaTeXe}{LaTeX2e}}
\abbrdef{mediabox}{/MediaBox}
\abbrdef{PD1}{PD1}
\abbrdef{pdf}{PDF}
\abbrdef{pdfdocencoding}{PDFDocEncoding}
\abbrdef{pdffile}{pdf file}
\abbrdef{pdfinfo}{\Program{pdfinfo}}
\abbrdef{pdfspec}{*pdf* specification}
\abbrdef{pdfstringdef}{\cms{pdfstringdef}}
\abbrdef{pdftex}{\Program{\pdfTeX}}
\abbrdef{perlscript}{perl script}
\abbrdef{plain}{plain}
\abbrdef{plaintex}{*plain*-*tex*}
\abbrdef{postscript}{PostScript}
\abbrdef{PU}{PU}
\abbrdef{sectioning}{section} % section?
\abbrdef{Sectioning}{Section}
\abbrdef{tex}{\TeX}
\abbrdef{texfile}{*tex* file}
\abbrdef{thumbpdf}{\Package{thumb\-pdf}}
\abbrdef{thumbpdf.pl}{\File{thumbpdf.pl}}
\abbrdef{toc}{\File{.toc}}
\abbrdef{unicode}{Unicode}
\abbrdef{winansiencoding}{WinAnsiEncoding}
\endinput


==> without review/hyperref/docinfo.tex <==
\foilhead[-\baselineskip]{General Document Information}

%\begin{Nav}{\NavInfo\NavBack}%
\begin{Nav}{\NavInfo}%
  \newcommand{\tit}[1]{%
    \multicolumn{2}{@{}l@{}}{\textbf{#1}}\\[0.5ex]%
  }
  \newcommand{\longentry}[1]{%
    \multicolumn{2}{@{}l@{}}{#1}%
  }
  \noindent
  Application: search engines.

  \noindent
  \begin{minipage}[t]{.55\linewidth}
    \begin{tabular}[t]{@{}l>{\tt}l@{}}
    \tit{\hypertarget{info}{*hyperref* options:}}%
    Title:&\Blue{pdftitle}\\
    Subject:&\Blue{pdfsubject}\\
    Author:&\Blue{pdfauthor}\\
    Keywords:&\Blue{pdfkeywords}\\
    Creator:&\Blue{pdfcreator}\\
    Producer:&\Blue{pdfproducer}
    \end{tabular}
  \end{minipage}%
  \begin{minipage}[t]{.45\linewidth}
    \begin{tabular}[t]{@{}ll@{}}
      \tit{Times:}%
      Created:&\Green{/CreationDate}\\
      Modificated:&\Green{/ModDate}\\[1ex]
      \tit{Informations:}%
      \longentry{File name, file size}\\
      \longentry{*pdf* version}\\
      \longentry{Optimized(linearized)}
    \end{tabular}
  \end{minipage}

  \subfoilhead{Setting\texorpdfstring{ the general document information}{}}
  \begin{smallpar}\hypertarget{infoanw}{}%
  \noindent
  \Code{\cms{usepackage}\{hyperref\}}\par
  \vspace{-\parskip}
  \catcode`\^^M=5
  \verbatiminput{pdfinfo}
  \end{smallpar}
  \newpage

\end{Nav}


\iffalse
\begingroup
  \makeatletter
  \def\hyper@anchorstart#1\hyper@anchorend{}%
  \pdfbookmark[1]{\file{hyperref} options}{optinfo}
\endgroup
\fi

\endinput


==> without review/hyperref/encoding.tex <==
\clearpage
\pdfbookmark[0]{Encodings}{enc}

\begingroup
\hypersetup{bookmarksopenlevel=2}


\subfoilhead[-\baselineskip]{Font encoding mechanism%
  \texorpdfstring{}{ of \abbr{latexe}}}

\noindent
\begin{tabular}{@{}l@{ }l@{ $\Rightarrow$ }l@{}}
plain-\TeX:& \code[green]<\ss>\ = \code[blue]<\char"19>&\Red{\ss}\\[1ex]
\LaTeXe:
  & \code<\fontencoding{OT1}\selectfont\char"19>&\Red{\ss}\\
  & \code<\fontencoding {T1}\selectfont\char"19>&\Red{\i}\\[0.5ex]
  & \code<\ss>\ = \code[blue]<\OT1-cmd \ss > \code[green]<\OT1\ss>&\Red{\ss}
\end{tabular}

\noindent
The font slot positions depend on the encoding:\\
\phantom{plain-\TeX: }\code[green]<\OT1\ss>\ = \code<\char"19>\\
\phantom{plain-\TeX: }\code[green]<\T1\ss>\phantom{\code<O>} =
  \code<\char"FF>\\
\phantom{plain-\TeX: }\code[green]<\?\ss>\phantom{\code<OT>} =
  \code<\UseTextSymbol{OT1}\ss>

%\begin{smallpar}
  \noindent
  \code<\> \code[blue]<OT1\ss>\ =
  \code<\csname > \code[blue]<OT1> \code<\string> \code[blue]<\ss>
    \code<\endcsname>
%\end{smallpar}


\subfoilhead[-\baselineskip]{PD1 encoding%
  \texorpdfstring{ (\abbr{pdfdocencoding})}{}}

\begin{itemize}
\def\1{\code[red]}%
\def\2{\code[blue]}\def\3{\Blue}%
\def\4#1{\Green{#1}\,=\,}%
\def\5{\Green}
\item Most names: \1<\text>%
    \3{\textsl{\textless glyph name\textgreater}}\\
    Examples:\quad
  \begin{tabular}[t]{@{}c@{\,=\,}l@{,\quad}c@{\,=\,}l@{}}
    \5\textregistered&\1<\text>\2<registered>&
    \5\textasciitilde&\1<\text>\2<asciitilde>
  \end{tabular}
\item Traditional *tex* and *latex* names.\\
    Examples:\quad
    \4\AE\2<\AE>,\quad
    \4\ss\2<\ss>
\item Accented characters.\\
    Examples:\quad
    \4{\"U}\2<\"U>,\quad
    \4{\c c}\2<\c c>,\quad
    \4{\r A}\2<\r A>~($\Leftarrow$\,\1<\AA>)
\item Escape octal sequences are the result:
%  \2<\textmu>\ (\Green{$\mu$}) $\Rightarrow$ \1<\265>
%  \2<\guillemotleft>\ (\Green{\guillemotleft}) $\Rightarrow$ \1<\253>
  \2<\textmu>\,$\Rightarrow$\,\1<\265>
\end{itemize}


\subfoilhead[-1.5\baselineskip]{PU encoding%
  \texorpdfstring{ (\abbr{unicode})}{}}

\begin{itemize}
\item[\frownie] Characters having catcodes 11 (letter) and 12 (other):\\
Checking each token, high memory and time consumption.
\item[\frownie] Ligatures: same as above.
\item[\frownie] Direct commands:\\
  Easier to implement, but each command must be redefined each time.
\item[\smiley] Commands of *latexe*'s fontencoding mechanism:\\
  Smallest memory consumption and fastest method.\\
  This method is used by package *hyperref*.
\end{itemize}


\subsubfoilhead[-\baselineskip]{Examples of \abbr{unicode} bookmarks}

\begingroup
\def\top#1{\vtop{\vskip0pt\hbox{#1}}}
\def\use#1{\top{\includegraphics[scale=1.2]{u0#1}}}
\centering
\begin{tabular}{@{}ll@{}}
\Blue{Greek}:&\Blue{Cyrillic}:\\
\use{3}&\use{4}\\
\end{tabular}
\par
\endgroup

\endgroup
\endinput


==> without review/hyperref/ende.tex <==
\clearpage
\pdfbookmark[0]{Ende}{ende}

\subfoilhead[-1.5\baselineskip]{Zusammenfassung}
\begin{itemize}
  \item \Red{Dokumenteninformation}:
    \begin{itemize}
      \item \file{hyperref}-Optionen in \code[blue]<\hypersetup>.
    \end{itemize}
  \item \Red{Lesezeichen}:
    \begin{itemize}
      \item Vorsicht wegen fehlender Magenverarbeitung
      \item Vieles durch \code[blue]<hyperref.sty>\ automatisiert.
      \item Zusatzpaket \code[blue]<hypbmsec.sty>
      \item Besondere Effekte erfordern "`low level"'-Eingriffe.
    \end{itemize}
  \item \Red{Thumbnails}:
    \begin{itemize}
      \item
      Einfache Benutzerschnittstelle mit \code[blue]<thumbpdf>.
    \end{itemize}
\end{itemize}


\subfoilhead[-\baselineskip]{Bezugsquellen}

\begin{smallpar}
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{PDF-Spezifikation}:\hfill
\url{http://www.adobe.com/supportservice/devrelations/PDFS/TN/PDFSPEC.PDF}\\[\sep]
  \it&\Blue{pdf\TeX}: \url{http://www.tug.org/applications/pdftex/}\\
  &Win32: \url{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}\\
  &Dokumantation: \url{http://www.pragma-ade.nl/pdftex.htm}\\[\sep]
  \it&\Blue{hyperref}, \Blue{pd1enc.def}, \Blue{hyparen.sty}:
\url{ftp://ftp.dante.de/tex-archive/macros/latex/contrib/supported/hyperref/}\\[\sep]
  \it&\Blue{hypbmsec}: Noch per E-Mail, CTAN geplant.\\[\sep]
  \it&\Blue{thumbpdf}:\hfill
\url{ftp://ftp.dante.de/tex-archive/macros/pdftex/thumbpdf/}\\[\sep]
  \it&\Blue{ghostscript}:
\url{http://www.cs.wisc.edu/~ghost/} oder\\&
\url{http://ftp.dante.de/tex-archive/support/ghostscript/aladdin/}
\end{tabularx}
\endgroup
\end{smallpar}

\rightfooter{%
  \ifprint
  \else
    \NavFull\NavSep\NavPrev\NavSep\NavQuit
  \fi
}


==> without review/hyperref/eurobm99.tex <==
%\includeonly{title,docinfo,strings,encoding,psd,hyperref,replace,pdfextra,thumb,summary,links,appendix}
%\includeonly{hyperref}

\begin{document}
\catcode`\*=\active
\include{title}
\include{docinfo}
\include{strings}
\include{encoding}
\include{psd}
\include{hyperref}
\include{replace}
\include{pdfextra}
\include{thumb}
\include{summary}
\include{links}
\include{appendix}
\end{document}


==> without review/hyperref/hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump



==> without review/hyperref/hyperref.tex <==
\foilhead{Bookmarks with package *hyperref*}
\begin{itemize}
\item Places for options.
\item Options for bookmarks.
\item Creating bookmarks.
\item Replacement methods.
\end{itemize}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead{Places for \texorpdfstring{*hyperref* }{}options}
\begin{enumerate}
\item Global: \Blue{\cms{documentclass}}\Code{[}\dots\Code{]} (*eg* driver)
\item Package: \Blue{\cms{usepackage}}\Code{[}\dots\Code{]}
\item Configuration file: \Blue{\File{hyperref.cfg}} with \cms{hypersetup}
\item After package has been loaded:
  \Blue{\cms{hypersetup}}\Code{\{}\dots\Code{\}}\\
  (*eg* *pdf* information options)
\end{enumerate}


\subfoilhead[-1.5\baselineskip]{Bookmark options}

\begingroup
  \def\sep{0.5ex}
  \noindent
  \Red{\Option{bookmarks}}: Make bookmarks
    (default: \Green{\Value{true}}).\\[\sep]
  \Red{\Option{bookmarksnumbered}}: Put section numbers in bookmarks
    (\Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopen}}: Open up bookmark tree
     (default: \Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopenlevel}}: Level, to which bookmarks are
     open.\\[\sep]
  \Red{\Option{pdfpagemode}}: How document starts when opened
     (default: \Green{\Value{None}}):
  \begingroup
    \mbox\qquad\Blue{\Option{None}}: Neither outlines nor thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{UseOutlines}}, \Blue{\Option{UseThumbs}}:
      Outlines, thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{FullScreen}}: Full-screen mode.\\[\sep]
  \endgroup
  \Red{\Option{unicode}}: Bookmarks in *unicode*
     (\Green{\Value{false}}). After package has been\\
     \mbox\qquad loaded, it switches between *unicode* and *pdfdocencoding*.
\endgroup


\subfoilhead[-0.5\baselineskip]{%
  \texorpdfstring{Bookmarks by \abbr{sectioning}}{\abbr{Sectioning}} %
  commands
}
\label{sec:bmbysec}

\begin{itemize}
\item Automatically addition of bookmarks by:
      \begin{itemize}
      \item \cms{part}, \cms{chapter}, \cms{section}, \cms{subsection}, \dots
      \item \cms{addcontentsline}
      \end{itemize}
\item Help file \Blue{\Code{\textsl{\cms{jobname}}.out}}:
      \begin{itemize}
      \item It is written in the \Green{first} run.
      \item The bookmarks are set in the \Green{second} run.
      \item There is \Green{\emph{no}} ``rerun'' warning.
      \end{itemize}
\end{itemize}


\subfoilhead{Tree structure\texorpdfstring{ of bookmarks}{}}

\begin{itemize}
\item Subentries must be added to \Blue{direct} ancestores,
      \Blue{not} grandparents.
\item If an intermediate level is omitted, the leaf starts \Blue{leftmost}:
      \begin{quote}
        \def\sub{\Red{\ensuremath{\rightarrow}}}%
        \def\ver{\Red{\ensuremath{\|}}}%
        \begin{tabular}{@{}lll@{}}
        &\Blue{table of contents}&\Blue{bookmarks}\\
        \hline
        \cms{part}\Code{\{I\}}&\ver{Part I}&\ver{main entry}\\
        \cms{chapter}\Code{\{5\}}&%
          \ver\sub{Chapter I.5}&\ver\sub{subentry}\\
        \cms{subsection}\Code{\{1\}}&
          \ver\sub\sub\sub{Subsection I.5.0.1}&\ver{main entry}\\
        \end{tabular}
      \end{quote}
\end{itemize}


\subfoilhead[-\baselineskip]{\texorpdfstring{Creating bookmarks with }{}\cms{pdfbookmark}}

\begin{itemize}
\item The bookmarks of *sectioning* commands have an \Red{level} number:
      \par\noindent
      \begin{tabular}{@{}lc@{ }c@{ }c@{ }c@{ }c@{}}
      documentclass&\cms{part}&\cms{chapter}&%
        \cms{section}&\cms{subsection}&\dots\\
      \Class{book}/\Class{report}:&\Red{\llap{$-$}1}&%
        \Red0&\Red1&\Red2&\dots\\
      \Class{article}:&\Red0&&\Red1&\Red2&\dots\\
      \end{tabular}
\item Syntax of \Blue{\cms{pdfbookmark}} (default for level: \Red{0}):
      \begin{quote}
        \Blue{\cms{pdfbookmark}}%
          \Code{[\Red{\emph{level}}]\{\emph{bookmark text}\}%
            \{\Green{\emph{anchor name}}\}}
      \end{quote}
\item \Blue{\cms{currentpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level}
\item \Blue{\cms{subpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level + 1}
\end{itemize}


\subsubfoilhead[-\baselineskip]{Using anchors%
  \texorpdfstring{ with \cms{pdfbookmark}}{}%
}

\begin{itemize}
\item An \Green{anchor name} consists of the argument and
      the level:
      \begin{quote}
        \Blue{\cms{pdfbookmark}}\Code{[\Red0]\{Titlepage\}\{\Green{tit}\}}%
          \Code{\commentchar\ }anchor: \Code{\Green{tit}.\Red0}
      \end{quote}
\item The bookmark can point to another \Green{target} (\Green{anchor}):
      \begin{quote}\small
        \cms{hypertarget}\Code{\{\Green{place.}\Red{1}\}\{\}}
      \end{quote}
      Redirecting the bookmark to the previous defined \Green{target}:
      \begin{quote}\small
        \cms{begingroup}\\
        *ind*\cms{makeatletter}\\
        *ind*\cms{def}\cms{hyper@anchorstart}\Code{ \#1}%
          \cms{hyper@anchorend}\Code{\{\}\%}\\
        *ind*\Blue{\cms{pdfbookmark}}\Code{[\Red1]\{Go to the place\}\{\Green{place}\}\%}\\
        \cms{endgroup}
      \end{quote}
\end{itemize}

\endgroup
\endinput


==> without review/hyperref/links.tex <==
\subfoilhead[-\baselineskip]{Links}

\begin{Nav}{\NavBookmarks\NavQuit}

\begin{smallpar}
\let\Blue\empty
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{*pdfspec*} (version 1.3):\newline
    \link{http://partners.adobe.com/asn/developer/PDFS/TN/PDFSPEC.PDF}%
    \tabularnewline[\sep]
  \it&\Blue{*pdftex*}:
    \begingroup
      \settoheight{\dimen0}{\mbox{\^e}}%
      \settoheight{\dimen1}{\mbox{e}}%
      \addtolength{\dimen0}{-\dimen1}%
    (H\`an Th\rlap{\raise\dimen0\hbox{\'{}}}\^e Th\`anh):
    \endgroup
    \newline
    \link{http://www.tug.org/applications/pdftex/}\newline
    Win32: \link{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}%
    \tabularnewline[\sep]
  \it&\Blue{*hyperref*} (Sebastian Rahtz):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/hyperref/}%
    \newline
    Test versions:\newline
    \link{http://www.tug.org/applications/hyperref/hyperref.zip}
    \tabularnewline[\sep]
  \it&\Blue{*hypbmsec*} (Heiko Oberdiek):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/oberdiek/}%
    \tabularnewline[\sep]
  \it&\Blue{*thumbpdf*} (Heiko Oberdiek):\newline
    \link{ftp://ctan.tug.org/tex-archive/macros/pdftex/thumbpdf/}%
\end{tabularx}
\endgroup
\end{smallpar}

%\SetNav{\NavFull\NavSep\NavPrev\NavSep\NavQuit}
\end{Nav}

\endinput


==> without review/hyperref/navbook.tex <==
\newcommand{\bmaction}[3][0]{%
  \begingroup
    \pdfstringdef\x{#3}%
    \pdfoutline user {<</S /Named /N /#2>>} count #1 {\x}%
  \endgroup
}
\bmaction[-3]{NOP}{Navigation}
  \bmaction[2]{FullScreen}{Full-screen}
    \bmaction{PageOnly}{Page only}
    \bmaction{ShowThumbs}{Thumbnails}
  \bmaction[6]{NOP}{Selecting pages}
    \bmaction{PrevPage}{Previous page}
    \bmaction{NextPage}{Next page}
    \bmaction{GoBack}{Go back}
    \bmaction{GoForward}{Go forward}
    \bmaction{FirstPage}{First page}
    \bmaction{LastPage}{Last page}
  \bmaction[2]{GeneralInfo}{General document information}
    \bmaction{ShowHideMenuBar}{Menu bar}
    \bmaction{ShowHideToolBar}{Tool bar}

\endinput


==> without review/hyperref/pdfextra.tex <==
\foilhead{Additional features of \abbr{pdf} format}
\noindent
Hyperref does not support all possibilities of *pdf* format, e.\,g.:
\begin{itemize}
  \let\Blue\empty
  \item \Blue{\Code{/CreationDate}} and \Blue{\Code{/ModDate}}.
  \item \Blue{Bookmarks} with \Blue{other functions}.
\end{itemize}
The following examples uses commands of \empty{*pdftex*}.

\subfoilhead{Bookmarks with other functions}
\begin{Nav}{\NavBookmarks\NavPage}

\begin{itemize}
  \item Menu functions of AcrobatReader, sound, video, \dots
  \item *pdftex* low level command:\\[1ex]
        \code[red]<\pdfoutline>\ \emph{\code<action>}\
        \code<count>\ \emph{\code[blue]<n>}\
        \code<{>\emph{\code<text>}\code<}>
        \begin{itemize}
          \item
            The absolute value of \emph{\code[blue]<n>}\ is the
            count of the direct subentries.
          \item
            If \emph{\code[blue]<n>}\ is negative, the
            subentries are closed.
        \end{itemize}
\end{itemize}


\subfoilhead{Link to external file}
\noindent
The *pdfspec* contains the possible actions on page 96.\\
At last a bookmark that points to that page:
\begingroup
  \edef\({\string(}
  \edef\){\string)}
\begin{verbatim}
$Blue(\pdfoutline)
  user {<<$Green(/S /GoToR /F $(pdfspec.pdf$) /D [95 /Fit])>>}
  count 0 {$empty(Description of actions)}
\end{verbatim}
\endgroup

\end{Nav}

\endinput


==> without review/hyperref/pdfinfo.tex <==
\hypersetup!{%
  pdftitle!    = {PDF information and navigation elements},
  pdfsubject!  = {Slides for talk at EuroTeX'99 in Heidelberg},
  pdfkeywords! = {pdf, hyperref, bookmarks, thumbnails},
  pdfauthor!   = {\textcopyright\ Heiko Oberdiek},
  pdfcreator!  = {\LaTeX\ with package \flqq hyperref\frqq},
  pdfproducer! = {pdfeTeX-0.\the\pdftexversion\pdftexrevision},
}
\pdfinfo!{/CreationDate! (D:19990909000000-01'00')}

==> without review/hyperref/psd.tex <==

\foilhead[-\baselineskip]{\cms{pdfstringdef}%
  \texorpdfstring{  converts \abbr{tex} to \abbr{pdf} strings}{}}

\noindent
Syntax: \Blue{\cms{pdfstringdef}}\Code{\{\emph{\cms{command}}\}%
    \{\emph{*tex* string}\}}

\begin{enumerate}
\item Selecting the encoding *PD1* or *PU*.
\item Redefinitions of many commands, so that they
      produce correct\\
      results or do not harm.
\item Expansion of the string.
\item Token checks and removal of forbidden tokens with 
      comprehensive\\ 
      warnings.
\end{enumerate}


\subfoilhead[-.5\baselineskip]{Redefinitions%
  \texorpdfstring{ by \cms{pdfstringdef}}{}}
\begin{itemize}
\item Redefinitions to get correct results, *eg*:
      \begin{itemize} 
      \item Glyph commands: \cms{\{}, \cms{\%}, \cms{space}, \cms{dots},
            \dots
      \item Logos: \cms{TeX}, \cms{LaTeX}, \cms{MF}, \dots
      \end{itemize}
\item Many tokens are removed silently, *eg*:
      \begin{itemize}
      \item *latex* commands: \cms{label}, \cms{index}, 
           \cms{textbf}, \dots
      \item Stomach tokens: curly group braces, \cms{relax} (\cms{protect}), 
            \dots
      \end{itemize}
\item The behaviour of \cms{xspace} is simulated.
\end{itemize}

\endinput


==> without review/hyperref/replace.tex <==
\foilhead{Replacement methods}

\begin{itemize}
%\item \code[blue]<\texorpdfstring>\ provides an alternative.
\item \Blue{\cms{texorpdfstring}} choices one of its arguments:\\
      a *tex* or a *pdf* string.
\item \code[blue]<\pdfstringdefPreHook>\ is a place for redefining commands.\\
      Additions are made by \code[blue]<\pdfstringdefDisableCommands>.
\item Package \Blue{*hypbmsec*} extends the \code<\section>\ commands.
\end{itemize}


\subfoilhead{\cms{texorpdfstring} method}
\noindent
Syntax: \Red{\cms{texorpdfstring}}%
        \Green{\Code{\{*tex* string\}}}%
        \Blue{\Code{\{*pdf* string\}}}

\noindent
Example:

\noindent
  \cms{section}\Code{\{}\Red{\cms{texorpdfstring}}%
  %\Code{\emph{\%}}%
  \Green{\Code{\{H\$\_2\$O\}}}%
  %\Code{\emph{\%}}%
  \Blue{\Code{\{Water\}}}%
  %\Code{\emph{\%}}%
  \Code{\}}


\subfoilhead[-1\baselineskip]{Hook for private macro redefinitions}

\begin{itemize}
\item \Red{\cms{pdfstringdefPreHook}} is called, before expanding the string.
\item \Red{\cms{pdfstringdefDisableCommands}} adds user redefinitions to\\
      \cms{pdfstringdefPreHook}

  \Blue{\cms{pdfstringdefDisableCommands}}\Code{\{\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{textcolor}\}[1]\{\#1\}\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{url}\}}\Code{\{}\empty{\cms{pdfstringdefwarn}}%
    \Code{\{\cms{url}\}}\Code{\}\commentchar}\\
  *ind*\cms{let}\cms{textcolor}\cms{@gobble}\\
  \Code{\}}
\item \Red{\cms{pdfstringdefwarn}} prints a warning message.
\end{itemize}


\subfoilhead[-\baselineskip]{Package \Package{hypbmsec}}

\begin{itemize}
\item The syntax of \cms{section} commands is extended:
      \begin{itemize}
      \item Second optional bookmark argument.
      \item Bookmark in parentheses.
      \end{itemize}
\item Syntax:
  \def\txt{\Blue{\textsl{text}}}%
  \def\toc{\Green{\textsl{toc/head}}}%
  \def\out{\Red{\textsl{bookmark}}}%
  \settowidth{\dimen0}{\toc}%
  \settowidth{\dimen1}{\out}%
  \addtolength{\dimen1}{-\dimen0}%
  \setlength{\dimen1}{.5\dimen1}%
  \edef\toc{\noexpand\Green{\noexpand\textsl{toc%
    \noexpand\hspace{\the\dimen1}/\noexpand\hspace{\the\dimen1}head}}}%
  \settowidth{\dimen0}{\textbf{]\{}}%
  \settowidth{\dimen1}{ = }%
  \addtolength{\dimen0}{-\dimen1}%
  \setlength{\dimen0}{-.5\dimen0}%
  \edef\xsp{\noexpand\hspace{\the\dimen0}}%
  \def\({\textbf{(}\,}%
  \def\){\,\textbf{)}}%
  \def\[{\textbf{[}\,}%
  \def\]{\,\textbf{]}}%
  \def\{{\textbf{\orgbraceleft}\,}%
  \def\}{\,\textbf{\orgbraceright}}%
  \def\section{\cms{section}}%
  \def~{ = }%
  \begin{tabular}[t]{@{}l@{ }c@{}c@{}c@{}c@{}c@{}l@{}}
    \section&\{&\toc&~&\out&~&\txt\}\\
    \section&\[&\toc&~&\out&\]\,\{&\txt\}\\[1ex]
    \section&\[&\toc&\]\,\[&\out&\]\,\{&\txt\}\\[1ex]
    \section&\(&\out&\)\,\{&\toc&~&\txt\}\\
    \section&\[&\toc&\]\,\(&\out&\)\,\{&\txt\}\\
    \section&\(&\out&\)\,\[&\toc&\]\,\{&\txt\}\\
  \end{tabular}
\end{itemize}


\endinput

The next version of package *hypbmsec* will know the
option \Blue{\Option{startotoc}}:
The starred *sectioning* commands are included in the table
of contents and in the outline tree automatically.
For options \Blue{\Option{infix}} and \Blue{\Option{prefix}}
see \secref{sec:addcontentsline}.

\endinput


==> without review/hyperref/strings.tex <==
\clearpage
\pdfbookmark[0]{Strings}{string}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead[-\baselineskip]{\abbr{pdf} strings}

\begin{itemize}
\item Examples, where *pdf* strings are used:
      \begin{quote}
      Bookmark names, information dictionaries, text annotations
      \end{quote}
\item *pdf* strings follow the *postscript* rules:
      \begin{itemize}
      \item Delimited by parentheses: \Code{\Blue{(}This is a string\Blue{)}}
      \item Escape sequences for white space, \Blue{\cms{(}}, \Blue{\cms{)}},
            \Blue{\cms{}\cms{}};\\
            octal notation, *eg*: `\"a\"o\"u\ss' = 
            \Code{(}\Blue{\cms{344}\cms{366}\cms{374}\cms{337}}\Code{)}
      \end{itemize}
\item 
%      $\vcenter{\mbox{%
        \begin{tabular}[t]{@{}l@{ }l@{}}
          \Blue{*pdfdocencoding*}:&8bit, superset of *isolatin1*\\
          \Blue{*unicode*}:&16bit, *acroread* version $\ge$ 4\\
        \end{tabular}%
%      }}$ 
\end{itemize}


\clearpage
\pdfbookmark[1]{\abbr{tex} strings}{strings}

\subsubfoilhead[-.5\baselineskip]{Digestion of \abbr{tex}}

\begingroup
\newenvironment{organ}[2]{%
  \begin{minipage}[t]{\linewidth}%
    \vspace{#2}%
    \begin{tabbing}%
      \begin{tabular}{@{\textbullet\ }l@{}}
        \multicolumn{1}{@{}l@{}}{%
%          \phantom{\textbullet\ }%
          \textbf{\large\Blue{#1}}}\\[0.5ex]
}{
      \end{tabular}%
    \end{tabbing}%
  \end{minipage}%
}

\makeatletter
\let\fbox\@firstofone

\noindent
\fbox{%
\begin{organ}{Eyes}{0pt}
  Reading input lines\\
  Catcodes are set
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Mouth}{2\baselineskip}
  Forming tokens\\
  Expansion of macros
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Stomach}{4\baselineskip}
  Assignments\\
  Typesetting
\end{organ}}%

\endgroup


\subsubfoilhead[-.5\baselineskip]{Differences between mouth and stomach}

\noindent
\begin{tabular}{@{}lll@{}}
  &\Blue{\textbf{mouth}}&
   \Blue{\textbf{stomach}}\\[1ex]
``zero'':& \code<\empty>&\code<\relax>\\[0.5ex]
\code<{...}>:&parameter&group\\[0.5ex]
variable:&read and check&assignments\\[0.5ex]
fonts:&--&different fonts and encodings\\
&&ligatures\\[0.5ex]
Commands:&\code<\string>, \code<\number>&\code<\def>, \code<\hbox>, \code<$>\\
&\code<\if>, \code<\the>&\code<\begingroup>, \code<\special>
\end{tabular}


\subfoilhead[-.5\baselineskip]{\abbr{tex} into \abbr{pdf} strings}

\begin{itemize}
\item Reusing the argument of *sectioning* commands (*tex* string)\\
      for the bookmarks (*pdf* strings).
\item Limitations because of missing stomach digestion:
      \begin{itemize}
      \item No manipulation of boxes, no mathematics, no colors, \dots
      \item No change of fonts or encodings, no ligatures.
      \item No assignments (\cms{xspace} uses \cms{futurelet}).
      \item Unexpandable commands appear verbatim.
      \end{itemize}
\end{itemize}


\endgroup
\endinput

==> without review/hyperref/summary.tex <==
\clearpage
\pdfbookmark[0]{End}{ende}

\subfoilhead[-1.5\baselineskip]{Summary}
\begin{itemize}
  \item \Red{General document information}:
    \begin{itemize}
      \item Options in \code[blue]<\hypersetup>\
            after \cms{usepackage}\Code{\{hyperref\}}.
    \end{itemize}
  \item \Red{Bookmarks}:
    \begin{itemize}
      \item Automatically added by \Blue{*hyperref*}.
      \item \Blue{Oral expansion}, no stomach commands (exceptions).
      \item Replacement methods: \code[blue]<\texorpdfstring>,\\
            \code[blue]<\pdfstringdefDisableCommands>, and
            \Blue{*hypbmsec*}.
      \item Low level commands only for special effects.
    \end{itemize}
  \item \Red{Thumbnails}: Automatically added by \Blue{*thumbpdf*}.
\end{itemize}


==> without review/hyperref/thumb.tex <==

\foilhead{Thumbnails}
\begin{Nav}{\NavThumbnails\NavBookmarks}
\thisthumb{zurueck}
\begin{itemize}
  \item Another method for navigation:
    \begin{itemize}
      \item Choosing pages.
      \item Selecting page areas.
    \end{itemize}
  \item Contents:
    \begin{itemize}
      \item Thumbnail sketches of the pages.
      \item Other pictograms, symbols, \dots
      \item Empty.
    \end{itemize}
\end{itemize}


\subfoilhead{Adding thumbnails with \abbr{thumbpdf}}
\thisthumb{weiter}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Nummer[#1]#2{\makebox(20,60)[#1]{%
    \vphantom{Hg}%
    $\smash{%
      \textsf{\textcircled{\vphantom{\large#2}\Blue{\small#2}}}%
    }$%
  }}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \begin{picture}(670,250)
    % Dateinamen
    \put(80,0){\FileBox{thumbdta.tex}}
    \put(80,100){\FileBox{\emph{jobname}.pdf}}
    \put(80,200){\FileBox{\emph{jobname}.tex}}
    \put(470,200){\FileBox{\Red{\emph{jobname}.pdf}}}
    % Pfeile
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(260,220){\line(1,0){210}}
    \put(470,220){\Right}
    \put(260,20){\line(1,0){105}}
    \put(365,20){\line(0,1){160}}
    \put(365,180){\Up}
    % Nummern
    \put(190,140){\Nummer[l]{1}}
    \put(190,40){\Nummer[l]{2}}
    \put(280,230){\Nummer[lb]{3}}
    % Programme
    \put(-10,40){\ProgBox[r]{*thumbpdf*}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(285,230){\ProgBox[b]{*pdftex*}}
    \put(285,150){\ProgBox[t]{\Code{thumbpdf.sty}}}
  \end{picture}
\endgroup

\subfoilhead[-\baselineskip]{How \abbr{thumbpdf} works}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \def\Left{\makebox(0,0)[l]{\LEFTarrow}}%
  \begin{picture}(650,340)
    % Dateinamen
    \put(80,0){\FileBox{\Red{thumbdta.tex}}}
    \put(80,100){\FileBox{thumbdta.pdf}}
    \put(80,200){\FileBox{thumb\emph{???}.png}}
    \put(80,300){\FileBox{\emph{jobname}.pdf}}
    \put(420,150){\FileBox{thumbopt.tex}}
    \put(420,240){\FileBox{\emph{other images}}}
    % Pfeile
    \put(170,300){\line(0,-1){60}}
    \put(170,240){\Down}
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(360,170){\line(1,0){60}}
    \put(360,170){\Left}
    \put(510,240){\line(0,-1){50}}
    \put(510,190){\Down}
    % Programme
    \put(-10,40){\ProgBox[r]{\textsf{perl}}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(190,140){\ProgBox[l]{\Code{thumbpdf.tex}}}
    \put(-10,240){\ProgBox[r]{*gs*}}
  \end{picture}
\endgroup


\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfoilhead{Thumbnails and *pdftex*}
\begin{itemize}
\item There is no direct support.
\item \code[blue]<\pdfimage> (*pdftex* versions below 0.14):
  \begin{itemize}
    \item[$+$] Image works as thumbnail.
    \item[$-$] No access to the image object number.
    \item[$-$] Image is on the page, must be
               moved out of the page.
  \end{itemize}
\item Low level commands
  \code[blue]<\pdfobj>\ and \code[blue]<\pdflastobj>\ are possible.
\end{itemize}

\clearpage
\pdfbookmark[1]{Project *thumbpdf*}{thumbpdf}
\subsubfoilhead[-\baselineskip]{Solution\texorpdfstring{ of project *thumbpdf*}{}}

\begin{enumerate}
  \item Generating the thumbnails \Blue{\file{thumb???.png}} by \Red{*gs*}.
  \item \Red{*pdftex*} runs \Red{\file{thumbpdf.tex}},
        thumbnails included by \code[blue]<\pdfimage>.
  \item The perl script \Red{\file{thumbpdf.pl}} reads
        \Blue{\file{thumbpdf.pdf}} and writes\\
        the object data in a *tex*
        readable form \Blue{\file{thumbdta.tex}}.
  \item Package \Red{\file{thumbpdf.sty}} inputs \Blue{\file{thumbdta.tex}},
        that contains the\\
        thumbnails as *pdf* objects (\code[blue]<\pdfobj>).
  \item The object numbers of the thumbnails (\code[blue]<\pdflastobj>)
        are added\\
        to the page attributes (\code[blue]<\pdfpageattr>).
\end{enumerate}


\subsubfoilhead[-.5\baselineskip]{User interface\texorpdfstring{ of *thumbpdf*}{}}

\begin{itemize}
  \def\master{\textsl{master}}%
  \item Command lines (\file{\master.tex} inputs \file{thumbpdf.sty}):
    \begin{enumerate}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
      \item \Blue{\texttt{thumbpdf \master}}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
    \end{enumerate}
  \item Another program than *gs* can be used:
    \begin{enumerate}
      \item[2a.] \Blue{\texttt{\textsl{ProgramThatGeneratesThumbnails} \master.pdf}}
      \item[2b.] \Blue{\texttt{thumbpdf}}
    \end{enumerate}
\end{itemize}

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subfoilhead[-\baselineskip]{Other images as thumbnails}

\begin{itemize}
\item With \Blue{\cms{thumb}} other images are declared as
      thumbnails in the\\ 
      optional file \Blue{\file{thumbopt.tex}}.
\item \Blue{\cms{thisthumb}} sets the thumbnail for the current page.
\end{itemize}
\begingroup
  \let\Red\Green
  \centering
  \begin{tabular}{@{}l@{\quad$\rightarrow$\quad}l@{}}
    \multicolumn{1}{@{}l}{\empty{\File{thumbopt.tex}}}&%
      \File{\emph{jobname}.tex}\\
    \hline
    \empty{\cms{thumb}}\Code{\{\Red{one}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
    \empty{\cms{thumb}}\Code{\{\Red{one.png}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one.png}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{two}]\{one\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{two}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{one}]\{./extras/one.png\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
  \end{tabular}
  \par
\endgroup

\end{Nav}

\endinput


==> without review/hyperref/thumbopt.tex <==
\thumb[zurueck]{addthumb/thumb001.png}
\thumb[weiter]{addthumb/thumb002.png}


==> without review/hyperref/title.tex <==
\pdfbookmark[0]{Beginning}{anfang}
\pdfbookmark[1]{Title}{title}

%\date{21st September 1999}% EuroTeX'99
\date{13rd October 1999}% first release for hyperref
\title{*pdf* information and navigation elements with
       hyperref, *pdftex*, and thumbpdf}
\author{Heiko Oberdiek\\\Email{oberdiek@ruf.uni-freiburg.de}}

\begingroup
  \LogoOff\aftergroup\LogoOn
  \Restriction{\unskip\centerline{\NavStart}}%
  \aftergroup\Restriction\aftergroup\empty
  \maketitle
  \begin{abstract}
    \noindent
    Additional possibilities for information and navigation through
    paper-less on-line documents that offer the PDF format.
  \end{abstract}
  \newpage
\endgroup

\subfoilhead{Subjects}
\begin{itemize}
\item General document information\hfill*hyperref*
\item Bookmarks/outlines\hfill*hyperref*
\item Thumbnails\hfill*thumbpdf*
\end{itemize}

\endinput

